Secrecy by Witness-Functions under Equational Theories

In this paper, we use the witness-functions to analyze cryptographic protocols for secrecy under nonempty equational theories. The witness-functions are safe metrics used to compute security. An analysis with a witness-function consists in making sure that the security of every atomic message does not decrease during its lifecycle in the protocol. The analysis gets more difficult under nonempty equational theories. Indeed, the intruder can take advantage of the algebraic properties of the cryptographic primitives to derive secrets. These properties arise from the use of mathematical functions, such as multiplication, addition, exclusive-or or modular exponentiation in the cryptosystems and the protocols. Here, we show how to use the witness-functions under nonempty equational theories and we run an analysis on the Needham-Schroeder-Lowe protocol under the cipher homomorphism. This analysis reveals that although this protocol is proved secure under the perfect encryption assumption, its security collapses under the homomorphic primitives. We show how the witness-functions help to illustrate an attack scenario on it and we propose an amended version to fix it.

==> Notations.tex <==
\section*{ Notations}
Hereafter, we give some definitions and conventions that will be used throughout the paper. 
\begin{itemize}
\item[+] We denote by  ${\cal{C}}=\langle{\cal{M}},\xi,\models,{\cal{K}},{\cal{L}}^\sqsupseteq,\ulcorner.\urcorner\rangle$ the context containing the parameters that affect the analysis of a protocol:
\begin{itemize}
\item[$\bullet$] ${\cal{M}}$ : is a set of messages built from the algebraic signature $\langle\cal{N}$,$\Sigma\rangle$ where ${\cal{N}}$ is a set of atomic names (nonces, keys, principals, etc.) and $\Sigma$ is a set of allowed functions ($enc$:\!: encryption\index{Encryption}, $dec$:\!: decryption\index{Décryption}, $pair$:\!: concatenation (denoted by "." here), etc.). i.e. ${\cal{M}}=T_{\langle{\cal{N}},\Sigma\rangle}({\cal{X}})$.  We use $\Gamma$ to denote the set of all possible substitution from $ {\cal{X}} \rightarrow {\cal{M}}$.
We denote by $\cal{A}$ all atomic messages in ${\cal{M}},$  by ${\cal{A}}(m)$ the set of atomic messages (or atoms) in $m$ and by ${\cal{I}}$ the set of agents (principals) including the intruder $I$. We denote by $k{^{-1}}$ the reverse key of a key $k$ and we consider that $({k^{-1}})^{-1}=k$.
\item[$\bullet$] $\xi$ : is the equational theory that describes the algebraic properties of the functions in $\Sigma$ by equations. e.g. $dec(enc(x,y),y^{-1})=x$. 
\item[$\bullet$] $\models$ : is the inference system of the intruder under the equational theory. Let $M$ be a set of messages and $m$ a message. $M$ $\models$ $m$ means that the intruder is able to infer $m$ from $M$ using her capacity. We extend this notation to traces as following: $\rho$ $\models$ $m$ means that the intruder can  infer $m$ from the messages exchanged in the trace $\rho$.
\item[$\bullet$] ${\cal{K}}$ : is a function from ${\cal{I}}$ to ${\cal{M}}$, that assigns to any agent (principal) a set of atomic messages describing her initial knowledge. We denote by $K_{{\cal{C}}}(I)$ the initial knowledge of the intruder, or simply $K(I)$ where the context is clear.
\item[$\bullet$] ${\cal{L}}^\sqsupseteq$ : is the security lattice $({\cal{L}},\sqsupseteq, \sqcup, \sqcap, \bot,\top)$ used to attribute security levels to  messages. 
A concrete example of a lattice is $ (2^{\cal{I}},\subseteq,\cap,\cup,\cal{I}, \emptyset)$ that will be used to attribute to a message $\alpha$ the set of principals that are allowed to know it. 
\item[$\bullet$] $\ulcorner .\urcorner$ : is a partial function that assigns a value of security (type) to a message in ${\cal{M}}$. Let $M$ be a set of messages and $m$ a message. We write $\ulcorner M \urcorner \sqsupseteq \ulcorner m \urcorner$ if
$\exists m' \in M. \ulcorner m' \urcorner \sqsupseteq \ulcorner m \urcorner$
%% \item[$\bullet$] 
\end{itemize}
\item[+] Let $p$ be a protocol, we denote by $R_G(p)$ the set of the generalized roles extracted from $p$. A generalized  role is  a  protocol abstraction  where  the emphasis is put on a particular principal and all the unknown messages are replaced by variables. More details about the role-based specification are in~\cite{Debbabi11,Debbabi22,Debbabi33}.
\begin{comment}
 Hereafter, an example of a protocol and its generalized roles.
 \begin{center}
  {\small
  \begin{tabular}{|ll|}
  \hline
  \hline
  \multicolumn{1}{|c} {Protocol $p$}& \multicolumn{1}{|c|}{$R_G(p)$}\\
  \hline
  \hline
   &$\begin{array}{llllll}
   \multicolumn{6}{c} { \mbox{Generalized role of } A}\\
    \alpha.1 & \textcolor{red}{A}    & \longrightarrow  & I(B) &:&  A\\
    \alpha.2 & I(B) &  \longrightarrow  & \textcolor{red}{A}   &:&  \textcolor{blue}{X}\\
    \alpha.3 & \textcolor{red}{A}    & \longrightarrow   & I(B) &:&  \{\textcolor{blue}{X}\}_{k_{as}}\\
    \end{array}$\\
 $\begin{array}{llllll}
    1 & A &  \longrightarrow & B &:&   A\\
    2 & B &  \longrightarrow  & A &:&   N_b\\
    3 & A &  \longrightarrow  & B &:&  \{N_b\}_{k_{as}}\\
    4 & B &  \longrightarrow  & S &:&  \{A.\{N_b\}_{k_{as}}\}_{k_{bs}}\\
    5 & S &  \longrightarrow  & B &:&  \{N_b\}_{k_{bs}}\\
    \end{array}$&
    $\begin{array}{llllll}
   \multicolumn{6}{c} { \mbox{Generalized role of } B}\\
    \alpha.1 & I(A) &  \longrightarrow  & \textcolor{red}{B}    &:&   A\\
    \alpha.2 & \textcolor{red}{B}    &  \longrightarrow  & I(A) &:&   N_b^\alpha\\
    \alpha.3 & I(A) &  \longrightarrow  & \textcolor{red}{B}   &:&  \textcolor{blue}{Y}\\
    \alpha.4 & \textcolor{red}{B}   &  \longrightarrow  & I(S) &:&  \{A.\textcolor{blue}{Y}\}_{k_{bs}}\\
    \alpha.5 & I(S) &  \longrightarrow  & \textcolor{red}{B}    &:&  \{N_b^\alpha\}_{k_{bs}}\\
    \end{array}$\\
    &$\begin{array}{llllll}
   \multicolumn{6}{c} { \mbox{Generalized role of } S}\\
    \alpha.4 & I(B) &  \longrightarrow  & \textcolor{red}{S}    &:&  \{A.\{\textcolor{blue}{Z}\}_{k_{as}}\}_{k_{bs}}\\
    \alpha.5 & \textcolor{red}{S}    &  \longrightarrow  & I(B) &:&  \{\textcolor{blue}{Z}\}_{k_{bs}}\\
    \end{array}$\\
    \hline
    \hline
    \end{tabular}}
 \end{center}
\end{comment}

We denote by ${\cal{M}}_p^{\cal{G}}$ the set of messages with variables generated by $R_G(p)$, by ${\cal{M}}_p$ the set of closed messages generated by substituting terms in ${\cal{M}}_p^{\cal{G}}$.  We denote by $R^+$ (respectively $R^-$) the set of sent messages (respectively received messages) by a honest agent in the role $R$. Commonly , we reserve the uppercase letters for sets or sequences of elements and the lowercase for single elements. For instance $M$ denotes a set of messages, $m$ a single message, $R$ a role composed of a sequence of steps, $r$ a step and $R.r$ the role ending by the step $r$.
\item[+] A valid trace is an interleaving of instantiated generalized roles where each message sent by the intruder can be produced by her using her capacity and the previous received messages. We denote by $ [\![p]\!]$ the set of valid traces of $p$.
\item[+] We assume that the intruder has the full-control of the net, as described in the Dolev-Yao model~\cite{DolevY1} with no restriction neither on the size of messages nor on the number of sessions.
\end{itemize}





%%We assume that the context of verification is also the same that in ~\cite{Houmani1,Houmani3,Houmani8,Houmani5} that we denote by ${\cal{C}}$.


==> WooLamCorrect.tex <==
\section{Analysis of the Woo-Lam Protocol (Amended Version) with a witness-function}\label{sectionAnWL2}

Here, we analyze an amended version of the Woo-Lam protocol with a witness-function and we prove that is correct for secrecy. This version  is  denoted by $p$ in Table~\ref{WLMV:protv2p}.

          \begin{table}[h]
         \caption{Woo-Lam Protocol-Amended version}
         \label{WLMV:protv2p} 
               \begin{center}$\begin{array}{|l|}
               \hline\\
                   \begin{array}{llll}
                    p   =&\langle 1,A\rightarrow B: A\rangle.  \\
                    & \langle 2,B\rightarrow A: N_b\rangle. \\
                    & \langle 3,A\rightarrow B: \{ B.k_{ab}\}_{k_{as}}\rangle. \\
                    & \langle 4,B\rightarrow S:\{A.N_b.\{B.k_{ab}\}_{k_{as}}\}_{k_{bs}}\rangle.  \\
                    & \langle 5,S\rightarrow B:\{N_b.\{A.k_{ab}\}_{k_{bs}} \}_{k_{bs}}\rangle\\ &\\
                    \end{array} \\ \hline  \end{array}$
         \end{center}

         \end{table}


    The   role-based   specification  of $p$  is ${\cal R}_G(p) = \{{\cal A}_G ^1,
    ~{\cal  A}_G  ^2,~{\cal B}_G ^1,~{\cal B}_G ^2,~{\cal B}_G ^3,~ {\cal S}_G ^1\}$,
    where the generalized roles ${\cal A}_G ^1$, ${\cal A}_G ^2$ of $A$ are as follows:
    \[\begin{array}{l}
            \begin{array}{lllll}
                    {\cal A}_G ^1 =& \langle  i.1, A    & \rightarrow & I(B):&  A
                    \rangle\\
            \end{array}\\
                    \\
             \begin{array}{llllll}
                    {\cal A}_G ^2=& \langle  i.1,  A    & \rightarrow & I(B):&  A \rangle .\\
                    & \langle i.2,  I(B) & \rightarrow & A:&  X \rangle .\\
                    & \langle i.3,  A    & \rightarrow & I(B):&  \{B.k_{ab}^i\}_{k_{as}}\rangle
             \end{array}\end{array}\]

     The generalized roles ${\cal B}_G ^1$, ${\cal B}_G ^2$, ${\cal B}_G
    ^3$  of $B$ are as follows:
            \[\begin{array}{l}
            \begin{array}{lllll}
                {\cal B}_G ^1=& \langle i.1,  I(A) & \rightarrow & B:&  A \rangle .\\
                        & \langle i.2,  B    & \rightarrow & I(A) :&  N_b^i \rangle  \\
            \end{array}\\ \\
            \begin{array}{lllll}
                    {\cal B}_G ^2=& \langle i.1,  I(A) & \rightarrow & B :&  A \rangle .\\
                    & \langle i.2,  B    & \rightarrow & I(A):&  N_b ^i\rangle .\\
                    & \langle i.3,  I(A) & \rightarrow & B:&  Y \rangle .\\
                    & \langle i.4,  B    & \rightarrow & I(S):& \{A.N_b^i.Y \}_{k_{bs}}\rangle
            \end{array}\\ \\
            \begin{array}{lllll}
                    {\cal B}_G ^3=& \langle i.1,  I(A) & \rightarrow & B:&  A \rangle .\\
                    & \langle i.2,  B    & \rightarrow & I(A):&  N_b ^i\rangle.\\
                    & \langle i.3,  I(A) & \rightarrow & B:&  Y \rangle.\\
                    & \langle i.4, B    & \rightarrow & I(S):& \{A.N_b^i.Y \}_{k_{bs}}\rangle.  \\
                    & \langle i.5,  I(S) & \rightarrow & B:&  \{N_b^i.\{A.Z\}_{k_{bs}}\}_{k_{bs}}\rangle \\
            \end{array}
             \end{array}\]

             The  generalized role $ {\cal S}_G ^1$ of $S$ is as follows:
            \[\begin{array}{l}
             \begin{array}{lllll}
                            {\cal S}_G ^1= & \langle i.4, I(B) & \rightarrow & S:& \{A.U.\{B.V\}_{k_{as}}
                            \}_{k_{bs}} \rangle. \\
                                    & \langle i.5,S & \rightarrow & I(B):& \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}\rangle\\
               \end{array}
            \end{array} \]
Let us have a context of verification such that: \\
$\ulcorner k_{as}\urcorner=\{A, S\}$; $\ulcorner k_{bs}\urcorner=\{B, S\}$; $\ulcorner k_{ab}^i\urcorner=\{A, B, S\}$; 
$\ulcorner N_b^i \urcorner=\bot$; $\forall A\in {\cal{I}}, \ulcorner A \urcorner=\bot$.\\
The principal identities are not analyzed since they are set public in the context.\\
Let $F= F_{MAX}^{EK}$; ${\cal{W}}_{p,F}= {\cal{W}}_{p,F_{MAX}^{EK}}$;\\
We denote  by ${\cal{W}}_{p,F}'(\alpha,m)$ the lower-bound $\underset{\overset {m' \in {\cal{M}}_p^{\cal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m\sigma' }}{\sqcap}\!\!\!\!\!\!\!\!\!\!  F(\alpha, \partial [\overline{\alpha}]m'\sigma')$ of the witness-function ${\cal{W}}_{p,F}(\alpha,m)$.\\
Let  ${\cal{M}}_p^{\cal{G}}=\{
A_1,
X_1,
\{B_1.K_{A_{2}B_{1}}^i\}_{K_{A_{2}S_{1}}},
A_3 ,
N_{B_{2}}^i,
Y_1,$\\$
\{A_4.N_{B_{3}}^i.Y_2 \}_{K_{{B_{3}S_2}}},
\{N_{B_{4}}^i.\{A_5.Z_1\}_{K_{B_{4}S_3}}\}_{K_{B_{4}S_3}},\\
\{A_6.U_1.\{B_5.V_1\}_{K_{{A_6}S_4}}\}_{K_{{B_5}S_4}},
\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}}
 \}$\\
After elimination of duplicates,
${\cal{M}}_p^{\cal{G}}=\\ \{
A_1,
X_1,
\{B_1.K_{A_{2}B_{1}}^i\}_{K_{A_{2}S_{1}}},
N_{B_{2}}^i,
\{A_4.N_{B_{3}}^i.Y_2 \}_{K_{{B_{3}S_2}}},$\\$
\{N_{B_{4}}^i.\{A_5.Z_1\}_{K_{B_{4}S_3}}\}_{K_{B_{4}S_3}},\\
\{A_6.U_1.\{B_5.V_1\}_{K_{{A_6}S_4}}\}_{K_{{B_5}S_4}},
\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}}
 \}$\\
The variables are denoted by $X_1, Y_2, Z_1, U_1, U_2, V_1$ and $V_2$;\\ 
The static names are denoted by $A_1$, $B_1$, $K_{A_{2}B_{1}}^i$, ${K_{A_{2}S_{1}}}$, 
$N_{B_{2}}^i$, $A_4$, $N_{B_{3}}^i$, ${K_{{B_{3}S_2}}}$, 
$N_{B_{4}}^i$, $A_5$, ${K_{B_{4}S_3}}$, 
$A_6$, $B_5$, ${K_{{A_6}S_4}}$, ${K_{{B_5}S_4}}$, 
$A_7$ and ${K_{B_{6}S_5}}$.

\subsection{Analysis of the Generalized Roles of $A$}
As defined in the generalized role $A$, an agent $A$ can participate in some session $S^{i}$  in which she receives an unkown message $X$ and sends the message $\{B.k_{ab}^i\}_{k_{as}}$. This is described by the following rule: \[{S^{i}}:\frac{X}{\{B.k_{ab}^i\}_{k_{as}}}\]

\noindent{-Analysis of the messages exchanged  in $S^{i}$:}\\
\\
1- For any $k_{ab}^i$:\\
\\
a- When receiving: $R_{S^{i}}^-=X$ \textit{(on receiving, we use the upper-bound)}\\
$F(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=F(k_{ab}^i,\epsilon)=\top$ (1.0)\\
\\
b- When sending: $r_{S^{i}}^+=\{B.k_{ab}^i\}_{k_{as}}$ \textit{(on sending, we use the lower-bound)}\\
 $\forall k_{ab}^i.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall k_{ab}^i.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{B.k_{ab}^i\}_{k_{as}}\sigma' } \}$ \\$=\{(\{B_1.K_{A_{2}B_{1}}^i\}_{K_{A_{2}S_{1}}},\sigma_1')\}$ such that: $ \sigma_1'=\{ B_1 \longmapsto B, K_{A_{2}B_{1}}^i \longmapsto k_{ab}^i, {K_{A_{2}S_{1}}} \longmapsto {k_{as}}\}$\\
${\cal{W}}_{p,F}'(k_{ab}^i,\{B.k_{ab}^i\}_{k_{as}})$\\
$=\{\mbox{Definition of the lower-bound of the witness-function}\}$\\
$F(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{B_1.K_{A_{2}B_{1}}^i\}_{K_{A_{2}S_{1}}} \sigma_{1}')$\\
$=\{\mbox{Extracting the static neighborhood}\}$\\
$F(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{B.k_{ab}^i\}_{k_{as}} \sigma_{1}')$ \\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
$F(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{B.k_{ab}^i\}_{k_{as}})$ \\
%%$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
$F(k_{ab}^i,\{B.k_{ab}^i\}_{k_{as}})$ \\
$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$\{B, A, S\}$(1.1)\\
\\
2- Compliance with the theorem \ref{PAT}:\\
From (1.0) and (1.1), we have: ${\cal{W}}_{p,F}'(k_{ab}^i,\{B.k_{ab}^i\}_{k_{as}})= \{A, B, S\} \sqsupseteq \ulcorner k_{ab}^i \urcorner \sqcap F(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=\{A, B, S\}$ (1.2)\\
From (1.2) we have: the messages exchanged in the session $S^{i}$ (i.e. $k_{ab}^i$) respect the theorem \ref{PAT}. (I)


\subsection{Analysis of the generalized roles of $B$}
As defined in the generalized roles of $B$, an agent $B$ can participate in two subsequent sessions: $S^{i}$ and $S^{j}$ such that $j>i$. In the former session $S^{i}$, the agent $B$ receives the identity $A$ and sends the nonce $N_b ^i$. In the subsequent session $S^{j}$, she receives an unknown message $Y$ and she sends the message $\{A.N_b^i.Y \}_{k_{bs}}$. This is described by the following rules:
\[{S^{i}}:\frac{A}{N_b ^i} ~~~~~~~~~~~~~~~~~~~~~~~~ {S^{j}}:\frac{Y}{\{A.N_b^i.Y \}_{k_{bs}}}\]
$ $\\
\noindent{-Analysis of the messages exchanged  in  $S^{i}$:}\\
\\
1- For any $N_b^i$:\\
Since $N_b^i$ is declared public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then we have directly:\\
${\cal{W}}_{p,F}'(N_b^i,N_b^i)\sqsupseteq \ulcorner N_b^i \urcorner \sqcap F(N_b^i,\partial  [\overline{N_b^i}]A )=\bot$ (2.1)\\
\\
\noindent{-Analysis of the messages exchanged  in $S^{j}$:}\\
\\
1- For any $N_b^i$:\\
Since $N_b^i$ is declared public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then we have directly:\\
${\cal{W}}_{p,F}'(N_b^i,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner N_b^i \urcorner \sqcap  F(N_b^i,\partial  [\overline{N_b^i}]Y )=\bot$ (2.2)\\
\\
2- For any $Y$:\\
Since when receiving, we have $F(Y,\partial  [\overline{Y}]Y )=F(Y,Y)=\bot$, then we have directly:\\
${\cal{W}}_{p,F}'(Y,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner Y \urcorner \sqcap F(Y,\partial  [\overline{Y}]Y )=\bot$ (2.3)\\
\\
3- Compliance with the theorem \ref{PAT}:\\
From (2.1), (2.2) and (2.3) we have: the messages exchanged in the session $S^{i}$ and $S^{j}$  respect the theorem \ref{PAT}. (II)

\subsection{Analysis of the generalized roles of $S$}
As defined in the generalized role $S$, an agent $S$ can participate in some session $S^{i}$  in which she receives the message $ \{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}$ and sends the message $ \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}$. This is described by the following rule: \[{S^{i}}:\frac{\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}}{ \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}}\]
1- For any $U$:\\
\\
b- When receiving: $R_{S^{i}}^-=\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(on receiving, we use the upper-bound)}\\
$F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )=$\\$F(U,\{A.U.\{B\}_{k_{as}}\}_{k_{bs}} )=\{A, B, S\}$ (3.2)\\
\\
b-When sending: $r_{S^{i}}^+=\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}$ \textit{(on sending, we use the lower-bound)}\\
 $\forall U.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall U.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}} \sigma' } \}$ \\$=\{(\{\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}},\sigma_1')\}$ such that: $\sigma_1'=\{ U_2 \longmapsto U, A_7\longmapsto A, V_2 \longmapsto V, {K_{B_{6}S_5}}\longmapsto  {k_{bs}}\}$\\
\\
${\cal{W}}_{p,F}'(U,\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower-bound of the witness-function}\}$\\
$F(U,\partial[\overline{U}]\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}} \sigma_{1}') $\\
$=\{\mbox{Extracting the static neighborhood}\}$\\
$F(U,\partial[\overline{U}] \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}} \sigma_{1}')$ \\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
$F(U,\partial[\overline{U}] \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}})$ \\
%%$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
$F(U,\{U.\{A\}_{k_{bs}}\}_{k_{bs}})$ \\
$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$\{A, B, S\}$(3.2)\\
\\
2- For any $V$:\\
\\
a- When receiving: $R_{S^{i}}^-=\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(on receiving, we use the upper-bound)}\\
$F(V,\partial  [\overline{V}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}})=$\\$F(V,\{A.\{B.V\}_{k_{as}}\}_{k_{bs}} )=$ \\$\left\{
    \begin{array}{ll}
        \{A, B, S\} & \mbox{if } k_{as} \mbox{ is the external protective key} \\
                          & \mbox{of } V \mbox{ in } \{A.\{B.V\}_{k_{as}}\}_{k_{bs}} \\
                          \\
        \{A, B, S\} & \mbox{if } k_{bs} \mbox{ is the external protective key} \\
                          & \mbox{of } V \mbox{ in } \{A.\{B.V\}_{k_{as}}\}_{k_{bs}} 
   \end{array}=
\right.$ $\{A, B, S\}$
 (3.3)\\
\\
b-When sending: $r_{S^{i}}^+=\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}$ \textit{(on sending, we use the lower-bound)}\\
 $\forall V.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall V.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}} \sigma' } \}$ \\$=\{(\{\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}},\sigma_1'),$\\$(\{N_{B_{4}}^i.\{A_5.Z_1\}_{K_{B_{4}S_3}}\}_{K_{B_{4}S_3}},\sigma_2')\}$ such that:
$$\left\{
    \begin{array}{l}
      \sigma_1'=\{ U_2 \longmapsto U, A_7\longmapsto A, V_2 \longmapsto V, {K_{B_{6}S_5}}\longmapsto  {k_{bs}}\}   \\
      \sigma_2'=\{ U \longmapsto N_{B_{4}}^i, A_5\longmapsto A, Z_1 \longmapsto V, {K_{B_{4}S_3}}\longmapsto  {k_{bs}}\}  \\
    \end{array}
\right.$$
${\cal{W}}_{p,F}'(V,\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower-bound of the witness-function}\}$\\
$F(V,\partial[\overline{V}]\{U_2.\{A_7.V_2\}_{K_{B_{6}S_5}}\}_{K_{B_{6}S_5}} \sigma_{1}') \sqcap$\\$ F(V,\partial[\overline{V}]\{N_{B_{4}}^i.\{A_5.Z_1\}_{K_{B_{4}S_3}}\}_{K_{B_{4}S_3}} \sigma_{2}') $\\
$=\{\mbox{Extracting the static neighborhood}\}$\\
$F(V,\partial[\overline{V}] \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}} \sigma_{1}')\sqcap$\\$ F(V,\partial[\overline{V}] \{ N_{B_{4}}^i.\{A.V\}_{k_{bs}}\}_{k_{bs}} \sigma_{2}')$ \\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
$F(V,\partial[\overline{V}] \{U.\{A.V\}_{k_{bs}}\}_{k_{bs}}) \sqcap $\\$F(V,\partial[\overline{V}] \{N_{B_{4}}^i.\{A.V\}_{k_{bs}}\}_{k_{bs}})$ \\
%%$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
$F(V,\{\{A.V\}_{k_{bs}}\}_{k_{bs}}) \sqcap F(V,\{N_{B_{4}}^i.\{A.V\}_{k_{bs}}\}_{k_{bs}})$ \\
$=\{\mbox{Since } F=F_{MAX}^{EK}\}$\\
$\{ A, B, S\}$(3.4)\\
\\
3- Compliance with the theorem \ref{PAT}:\\
\\
For any $U$, from (3.1) and (3.2) we have:\\
${\cal{W}}_{p,F}'(U,\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}})=\{A, B, S\}\sqsupseteq \ulcorner U \urcorner \sqcap F(U,\partial  [\overline{U}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )=\ulcorner U \urcorner \cup \{A, B, S\}$ (3.5)\\
For any $V$, from (3.3) and (3.4) we have:\\
${\cal{W}}_{p,F}'(V,\{U.\{A.V\}_{k_{bs}}\}_{k_{bs}})=\{A, B, S\}\sqsupseteq \ulcorner V \urcorner \sqcap F(V,\partial  [\overline{V}]\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}} )=\ulcorner V \urcorner \cup \{A, B, S\}$ (3.6)\\
From (3.5)  and (3.6) we have: the messages exchanged in the session $S^{i}$  respect the theorem \ref{PAT} (III)

\section{Results and Interpretation}

The results of analysis of the amended version of the Woo-Lam protocol are summarized in Table \ref{WLAMGrowth}. From Table \ref{WLAMGrowth}, we conclude that this version fully respects the theorem \ref{PAT}. Hence, this protocol keeps its secrect inputs.

\begin{table}[h]
\caption{Compliance of the Woo-Lam protocol (amended version) with the Theorem \ref{PAT}}
\label{WLAMGrowth} 
   \centering
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
&  $\alpha$ &Role& $R^-$ & $r^+$ &  The.\ref{PAT}\\
  \hline
1&  $k_{ab}^i$ & $A$& $X$ & $\{B.k_{ab}^i\}_{k_{as}}$ & Ok\\
  \hline
2& $X$ &  $A$ & $X$ & $\{B.k_{ab}^i\}_{k_{as}}$& Ok\\
  \hline
 \hline
3&  $N_b^i$ & $B$& $A$ & $N_b^i$ & Ok\\
  \hline
4& $Y$ &  $B$ & $Y$ & $\{A.N_b^i.Y \}_{k_{bs}}$& Ok\\
  \hline
5& $N_b^i$ &  $B$ & $Y$ & $\{A.N_b^i.Y \}_{k_{bs}}$& Ok\\
  \hline
 \hline
6&  $U$ & $S$& $\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}$ & $\{A.V\}_{k_{bs}}\}_{k_{bs}}$ & Ok\\
  \hline
7& $V$ &  $S$ & $\{A.U.\{B.V\}_{k_{as}}\}_{k_{bs}}$ & $\{A.V\}_{k_{bs}}\}_{k_{bs}}$&  Ok\\
 \hline
\end{tabular}
\\\hspace{\linewidth}

\end{table}


==> WooLamFaille1.tex <==
\section*{Analysis of the Woo- Lam Protocol (Falwed Version) with a Witness-Function-First Essay}\label{sectionAnWL1}
In this section, we run an analysis on the flawed version of the Woo-Lam protocol using the Witness-Function ${{\cal{W}}}_{p,{F}_{N}^{EK}}$.
This version of the this protocol is denoted by $p$ in Table~\ref{WLMV:protv2p}.
          \begin{table}[h]
               \begin{center}$\begin{array}{|l|}
               \hline\\
                   \begin{array}{llll}
                    p   =&\langle 1,A\rightarrow B: A\rangle.  \\
                    & \langle 2,B\rightarrow A: N_b\rangle. \\
                    & \langle 3,A\rightarrow B: \{ N_b.k_{ab}\}_{k_{as}}\rangle. \\
                    & \langle 4,B\rightarrow S:\{A.\{N_b.k_{ab}\}_{k_{as}}\}_{k_{bs}}\rangle.  \\
                    & \langle 5,S\rightarrow B:\{N_b.k_{ab}\}_{k_{bs}}\rangle\\ &\\
                    \end{array} \\  \hline  \end{array}$
         \end{center}
    \caption{\label{WLMV:protv2p} The Woo and Lam Protocol (Flawed Version)}
         \end{table}

    The   role-based   specification   is ${\mathcal R}_G(p) = \{{\mathcal A}_G ^1,
    ~{\mathcal  A}_G  ^2,~{\mathcal B}_G ^1,~{\mathcal B}_G ^2,~{\mathcal B}_G ^3,~ {\mathcal S}_G ^1\}$,
    where the generalized roles ${\mathcal A}_G ^1$, ${\mathcal A}_G ^2$, of $A$ are as follows:
    \[\begin{array}{l}
            \begin{array}{lllllll}
                    {\mathcal A}_G ^1 =& \langle  i.1,&  A    & \rightarrow & I(B)&  :&  A
                    \rangle\\
            \end{array}\\
                    \\
             \begin{array}{lllllll}
                    {\mathcal A}_G ^2=& \langle  i.1,&  A    & \rightarrow & I(B)&  :&  A \rangle .\\
                    & \langle i.2,&  I(B) & \rightarrow & A   &  :&  X \rangle .\\
                    & \langle i.3,&  A    & \rightarrow & I(B)&  :&  \{X.k_{ab}^i\}_{k_{as}}\rangle
             \end{array}\end{array}\]

     The generalized roles ${\mathcal B}_G ^1$, ${\mathcal B}_G ^2$, ${\mathcal B}_G
    ^3$,  of $B$ are as follows:
            \[\begin{array}{l}
            \begin{array}{lllllll}
                {\mathcal B}_G ^1=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                        & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b^i \rangle  \\
            \end{array}\\ \\
            \begin{array}{lllllll}
                    {\mathcal B}_G ^2=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                    & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b ^i\rangle .\\
                    & \langle i.3,&  I(A) & \rightarrow & B   &  :&  Y \rangle .\\
                    & \langle i.4,&  B    & \rightarrow & I(S)&  :& \{A.Y \}_{k_{bs}}\rangle .
            \end{array}\\ \\
            \begin{array}{lllllll}
                    {\mathcal B}_G ^2=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                    & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b ^i\rangle .\\
                    & \langle i.3,&  I(A) & \rightarrow & B   &  :&  Y \rangle .\\
                    & \langle i.4,&  B    & \rightarrow & I(S)&  :& \{A.Y \}_{k_{bs}}\rangle .\\
                    & \langle i.5,&  I(S) & \rightarrow & B&  :&  \{{N_b^i}.Z\}_{k_{bs}} \rangle \\
            \end{array}
             \end{array}\]

             The  generalized role $ {\mathcal S}_G ^1$, of $S$ is as follows:
            \[\begin{array}{l}
             \begin{array}{lllllll}
                            {\mathcal S}_G ^1= & \langle i.4,& I(B) & \rightarrow & S & :&\{A.\{U.V\}_{k_{as}}\}_{k_{bs}} \rangle . \\
                                    & \langle i.5,& S & \rightarrow & I(B)& :& \{U.V\}_{k_{bs}}\rangle\\
               \end{array}
            \end{array} \]
Let us have a context of verification such that: \\
$\ulcorner k_{as}\urcorner=\{A, S\}$; $\ulcorner k_{bs}\urcorner=\{B, S\}$; $\ulcorner k_{ab}^i\urcorner=\{A, B, S\}$; 
$\ulcorner N_b^i \urcorner=\bot$; $\forall A\in {\mathcal{I}}, \ulcorner A \urcorner=\bot$.\\
The principal identities are not analyzed since they are set public in the context.\\
Let ${F} \equiv {F}_{N}^{EK}$; ${{\cal{W}}}_{p,{F}}\equiv {{\cal{W}}}_{p,{F}_{N}^{EK}}$;\\
We denote  by ${{\cal{W}}}_{p,{F}}'(\alpha,m)$ the lower bound: $\underset{\overset {m' \in {\mathcal{M}}_p^{\mathcal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m\sigma' }}{\sqcap} {F}(\alpha, \partial [\overline{\alpha}]m'\sigma')$ of the Witness-Function ${{\cal{W}}}_{p,{F}}(\alpha,m)$.\\
Let  ${\mathcal{M}}_p^{\mathcal{G}}=\{
A_1,
X_1,
\{X_2.k_{A_2 B_1}^i\}_{k_{A_2 S_1}},
A_3,\\
N_{B_{2}}^i,
Y_1,
 \{A_4.Y_1 \}_{k_{B_3 S_2}},
\{{N_{B_4}^i}.Z_1\}_{k_{B_4 S_3}},\\
\{A_5.\{U_1.V_1\}_{k_{A_5 S_4}}\}_{k_{B_5 S_4}},
\{U_2.V_2\}_{k_{B_6 S_5}}
 \}$\\
After elimination of duplicates,
${\mathcal{M}}_p^{\mathcal{G}}=\{
A_1,
X_1,
\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}},
N_{B_{2}}^i,
 \{A_4.Y_1 \}_{K_{B_3 S_2}},\\
\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},
\{A_5.\{U_1.V_1\}_{K_{A_5 S_4}}\}_{K_{B_5 S_4}},
\{U_2.V_2\}_{K_{B_6 S_5}}
 \}$\\The variables are denoted by $X_1, X_2,Y_1, Z_1, U_1, U_2, V_1$ and $V_2$;\\ 
The static names are denoted by $A_1$, $A_2$, $B_{1}$, ${K_{A_{2}S_{1}}}$, 
$N_{B_{2}}^i$, $A_4$, ${K_{{B_{3}S_2}}}$, 
$N_{B_{4}}^i$, ${K_{B_{4}S_3}}$, 
$A_5$, ${K_{{A_5}S_4}}$, ${K_{{B_5}S_4}}$ 
 and ${K_{B_{6}S_5}}$.
\subsection{Analysis of the generalized role of $A$}
As defined in the generalized role $A$, an agent $A$ can participate in some session $S^{i}$  in which she receives an unknown message $X$ and sends the message $\{X.k_{ab}^i\}_{k_{as}}$. This is described by the following schema: \[{S^{i}}:\frac{X}{\{X.k_{ab}^i\}_{k_{as}}}\]

\noindent\textbf{-Analysis of the messages exchanged  in the session $S^{i}$:}\\
\\
1- For any $k_{ab}^i$:\\
\\
a- When receiving: $R_{S^{i}}^-=X$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=\top$ (1.0)\\
\\
b- When sending: $r_{S^{i}}^+=\{X.k_{ab}^i\}_{k_{as}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall k_{ab}^i.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall k_{ab}^i.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{X.k_{ab}^i\}_{k_{as}}\sigma' } \}$ \\$=\{(\{X_2.K_{A_2 B_1}^i\}_{K_{A_2 S_1}},\sigma_1'), ( \{A_4.Y_1 \}_{K_{B_3 S_2}},\sigma_2'),$\\$(\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},\sigma_3'),(\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_4')\}$\\  such that: 
$$\left\{
    \begin{array}{l}
%%      \sigma_1'=\{X_1 \longmapsto\{X.k_{ab}^i\}_{k_{as}}\}   \\
      \sigma_1'=  \{X_2 \longmapsto X, K_{A_2 B_1}\longmapsto k_{ab}, {K_{A_2 S_1}} \longmapsto {k_{as}}\}\\
      \sigma_2'=  \{X\longmapsto A_4,Y_1 \longmapsto k_{ab}^i, K_{A_2 S_1} \longmapsto k_{as}\}\\
      \sigma_3'=  \{X\longmapsto {N_{B_4}^i},Z_1 \longmapsto k_{ab}^i, K_{B_4 S_3}\longmapsto k_{as}\}\\
      \sigma_4'=  \{U_2\longmapsto X,V_2 \longmapsto k_{ab}^i, K_{B_6 S_5}\longmapsto k_{as}\}\\
    \end{array}
\right.$$
${{\cal{W}}}_{p,{F}}'(k_{ab}^i,\{X.k_{ab}^i\}_{k_{as}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.K_{A_2 B_1}^i\}_{K_{A_2 S_1}} \sigma_{1}') \sqcap {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{A_4.Y_1 \}_{K_{B_3 S_2}} \sigma_{2}')\sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}} \sigma_{3}') \sqcap $\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{4}')$\\
$=\{\mbox{renaming the static neighborhood}\}$\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.k_{ab}^i\}_{k_{as}} \sigma_{1}') \sqcap {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{A_4.Y_1\}_{k_{as}} \sigma_{2}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{{N_{B_4}^i}.Z_1\}_{k_{as}} \sigma_{3}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{U_2.V_2\}_{k_{as}} \sigma_{4}')$   \\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.k_{ab}^i\}_{k_{as}}) \sqcap {F}(Y_1,\partial[\overline{Y_1}] \{A_4.Y_1\}_{k_{as}}) \sqcap $\\${F}(Z_1,\partial[\overline{Z_1}] \{{N_{B_4}^i}.Z_1\}_{k_{as}}) \sqcap {F}(V_2,\partial[\overline{V_2}] \{U_2.V_2\}_{k_{as}})$  \\
%%$=\{\mbox{Since } F=F_{N}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(k_{ab}^i,\{k_{ab}^i\}_{k_{as}}) \sqcap {F}(Y_1,\{A_4.Y_1\}_{k_{as}}) \sqcap {F}(Z_1,\partial[\overline{Z_1}] \{{N_{B_4}^i}.Z_1\}_{k_{as}}) \sqcap {F}(V_2,\partial[\overline{V_2}] \{V_2\}_{k_{as}})$ \\
$=\{\mbox{Since } {F}={F}_{N}^{EK}\}$\\
$\emptyset \cup \{A_4\} \cup \emptyset \cup \emptyset=\{A_4\}$(1.1)\\
\\
2- For any $X$:\\
\\
Since when receiving, we have ${F}(X,\partial  [\overline{X}]X )={F}(X,X)=\bot$, then we have directly:\\
${{\cal{W}}}_{p,{F}}'(X,\{X.k_{ab}^i\}_{k_{as}})\sqsupseteq \ulcorner X \urcorner \sqcap {F}(X,\partial  [\overline{X}]X)=\bot$ (1.2)\\
\\
3- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
From (1.0) and (1.1), we have: ${{\cal{W}}}_{p,{F}}'(k_{ab}^i,\{X.k_{ab}^i\}_{k_{as}})= \{A_4\} \not\sqsupseteq \ulcorner k_{ab}^i \urcorner \sqcap {F}(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=\{S, A, B\}$ (1.3)\\
From (1.3) we have: the messages exchanged in the session $S^{i}$ (i.e. $k_{ab}^i$) do not respect the correctness criterion stated in the theorem \ref{PAT}. (I)


\subsection{Analysis of the generalized role of $B$}
As defined in the generalized roles of $B$, an agent $B$ can participate in two consequent sessions: $S^{i}$ and $S^{j}$ such that $j>i$. In the former session $S^{i}$, the agent $B$ receives the identity $A$ and sends the nonce $N_b ^i$. In the consequent session $S^{j}$, she receives an unknown message $Y$ and she sends the message $\{A.N_b^i.Y \}_{k_{bs}}$. This is described by the following schema:
\[{S^{i}}:\frac{A}{N_b ^i} ~~~~~~~~~~~~~~~~~~~~~~~~ {S^{j}}:\frac{Y}{\{A.Y \}_{k_{bs}}}\]
$ $\\
\textbf{-Analysis of the messages exchanged  in the session $S^{i}$:}\\
\\
1- For any $N_b^i$:\\
Since $N_b^i$ is declared public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then we have directly:\\
${{\cal{W}}}_{p,{F}}'(N_b^i,N_b^i)\sqsupseteq \ulcorner N_b^i \urcorner \sqcap {F}(N_b^i,\partial  [\overline{N_b^i}]A )=\bot$ (2.1)\\
\\
\textbf{-Analysis of the messages exchanged  in the session $S^{j}$:}\\
\\
1- For any $Y$:\\
Since when receiving, we have ${F}(Y,\partial  [\overline{Y}]Y )={F}(Y,Y)=\bot$, then we have directly:\\
${{\cal{W}}}_{p,{F}}'(Y,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner Y \urcorner \sqcap {F}(Y,\partial  [\overline{Y}]Y )=\bot$ (2.2)\\
\\
2- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
From (2.1) and (2.2) we have: the messages exchanged in the session $S^{i}$ and $S^{j}$  respect the correctness criterion stated in the theorem \ref{PAT}. (II)

\subsection{Analysis of the generalized role of $S$}
As defined in the generalized role $S$, an agent $S$ can participate in some session $S^{i}$  in which she receives the message $ \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ and sends the message $\{U.V\}_{k_{bs}}$. This is described by the following schema: \[{S^{i}}:\frac{\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}}{\{U.V\}_{k_{bs}}}\]
1- For any $U$:\\
\\
a- When receiving: $R_{S^{i}}^-=\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}} )={F}(U,\{A.\{U\}_{k_{as}}\}_{k_{bs}} )=$\\$\left\{
    \begin{array}{ll}
        \{A\} & \mbox{if } k_{bs} \mbox{ is the EPK\footnote{External Protective Key} of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.1.1)\\
        \emptyset & \mbox{if } k_{as} \mbox{ is the EPK of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.1.2)
    \end{array}
\right.$ (3.1)\\
\\
b-When sending: $r_{S^{i}}^+=\{U.V\}_{k_{bs}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall U.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall U.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{U.V\}_{k_{bs}} \sigma' } \}$ \\$=\{\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}},\sigma_1'),(,\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_2')\}$ such that: \\
$$\left\{
    \begin{array}{l}
      \sigma_1'=\{ X_2 \longmapsto U,  V \longmapsto k_{A_2 B_1}^i, {K_{A_2 S_1}}\longmapsto  {k_{bs}}\}   \\
      \sigma_2'=\{ U_2 \longmapsto U, V_2\longmapsto V, K_{B_6 S_5}\longmapsto  {k_{bs}}\}  \\
    \end{array}
\right.$$
\\
${{\cal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(U,\partial[\overline{U}]\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}} \sigma_{1}') \sqcap {F}(U,\partial[\overline{U}]\{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{2}')$\\
$=\{\mbox{Setting the static neighborhood}\}$\\
${F}(U,\partial[\overline{U}]\{X_2.k_{A_2 B_1}^i\}_{k_{bs}} \sigma_{1}') \sqcap {F}(U,\partial[\overline{U}]\{U_2.V_2\}_{k_{bs}} \sigma_{2}')$
\\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(X_2,\partial[\overline{X_2}]\{X_2.k_{A_2 B_1}^i\}_{k_{bs}} \sigma_{1}') \sqcap {F}(U_2,\partial[\overline{U_2}]\{U_2.V_2\}_{k_{bs}} \sigma_{2}')$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(X_2,\{X_2.k_{A_2 B_1}^i\}_{k_{bs}}) \sqcap {F}(U_2,\{U_2\}_{k_{bs}})$ \\
$=\{\mbox{Since } {F}={F}_{N}^{EK}\}$\\
$\emptyset \cup \emptyset=\emptyset$ (3.2)\\
\\
2- For any $V$:\\
\\
a- When receiving: $R_{S^{i}}^-=\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})={F}(V,\{A.\{V\}_{k_{as}}\}_{k_{bs}})=$\\$\left\{
    \begin{array}{ll}
        \{A\} & \mbox{if } k_{bs} \mbox{ is the EPK of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.3.1)\\
        \emptyset & \mbox{if } k_{as} \mbox{ is the EPK of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.3.2)
    \end{array}
\right.$ (3.3)\\
\\
b-When sending: $r_{S^{i}}^+=\{U.V\}_{k_{bs}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall V.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall V.\{m' \in {\mathcal{M}}_p^{\mathcal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' =\{U.V\}_{k_{bs}} \sigma' } \}$ \\$=\{( \{A_4.Y_1 \}_{k_{B_3 S_2}},\sigma_1'),(\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},\sigma_2'),(\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_3')\}$ such that: \\
$$\left\{
    \begin{array}{l}
      \sigma_1'=\{ U \longmapsto A_4, Y_1 \longmapsto V, {K_{B_{3}S_2}}\longmapsto  {k_{bs}}\}   \\
      \sigma_2'=\{ U \longmapsto N_{B_{4}}^i, Z_1 \longmapsto V, {K_{B_{4}S_3}}\longmapsto  {k_{bs}}\}  \\
      \sigma_3'=\{ U_2 \longmapsto U, V_2 \longmapsto V, {K_{B_6 S_5}}\longmapsto  {k_{bs}}\}  \\
    \end{array}
\right.$$
\\
${{\cal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(V,\partial[\overline{V}] \{A_4.Y_1 \}_{k_{B_3 S_2}}\sigma_{1}') \sqcap {F}(V,\partial[\overline{V}]\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}} \sigma_{2}')\sqcap {F}(V,\partial[\overline{V}]\{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{3}')$\\
$=\{\mbox{Setting the static neighborhood}\}$\\
${F}(V,\partial[\overline{V}] \{A_4.Y_1\}_{k_{bs}}\sigma_{1}') \sqcap {F}(V,\partial[\overline{V}]\{{N_{B_4}^i}.Z_1\}_{k_{bs}} \sigma_{2}')\sqcap {F}(V,\partial[\overline{V}]\{U_2.V_2\}_{K_{bs}} \sigma_{3}')$\\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(Y_1,\partial[\overline{Y_1}] \{A_4.Y_1\}_{k_{bs}}\sigma_{1}') \sqcap {F}(Z_1,\partial[\overline{Z_1}]\{{N_{B_4}^i}.Z_1\}_{k_{bs}} \sigma_{2}')\sqcap {F}(V_2,\partial[\overline{V_2}]\{U_2.V_2\}_{K_{bs}} \sigma_{3}')$\\
%%$=\{\mbox{Since } F=F_{N}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(Y_1,\{A_4.Y_1\}_{k_{bs}}) \sqcap {F}(Z_1,\{{N_{B_4}^i}.Z_1\}_{k_{bs}})\sqcap {F}(V_2,\{V_2\}_{K_{bs}})$\\$=\{\mbox{Since } {F}={F}_{N}^{EK}\}$\\
$\{ A_4\}\cup \emptyset \cup \emptyset=\{ A_4\}$(3.4)\\
\\
3- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
For any $U$, from (3.1) and (3.2) we have:\\
%%\small{
\\$(3.5)  \left\{
  \begin{array}{ll}
 {{\cal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}}\}_{k_{bs}})=\emptyset \sqsupseteq& \\
\ulcorner U \urcorner \sqcap {F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=      \ulcorner U \urcorner \cup  \{A\} & \\
 \mbox{if } k_{bs} \mbox{ is the EPK of } U \mbox{ in } \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.5.1)&\\
\\
 {{\cal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}}\}_{k_{bs}})=\emptyset \sqsupseteq &\\
\ulcorner U \urcorner \sqcap {F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=     \ulcorner U \urcorner \cup   \emptyset& \\
\mbox{if } k_{as} \mbox{ is the EPK of } U \mbox{ in } \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.5.2)&\\
    \end{array}
\right.$ \\
$ $\\
%%}
\normalsize
For any $V$, from (3.3) and (3.4) we have:\\
%%\small{
\\$(3.6)\left\{
    \begin{array}{ll}
 {{\cal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})=\{A_4\} \not \sqsupseteq & \\
\ulcorner V \urcorner \sqcap {F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=   \ulcorner V \urcorner \cup     \{A, B, S\} &\\
\mbox{if } k_{bs} \mbox{ is the EPK of } V \mbox{ in } \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.6.1) &\\
\\
{{\cal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})=\{A_4\} \not\sqsupseteq &\\
\ulcorner V \urcorner \sqcap {F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=    \ulcorner V \urcorner \cup    \{A, S\}  & \\
\mbox{if } k_{as} \mbox{ is the EPK of } V \mbox{ in } \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.6.2) &\\
    \end{array}
\right.$ \\
%%}
\normalsize
$ $\\
From (3.6) we have: the messages exchanged in the session $S^{i}$  do not respect the correctness criterion stated in the theorem \ref{PAT} (III)

\section{Results and Interpretation}

The analysis results of the Woo and Lam protocol are summarized in Table \ref{WLAMGrowthFaille}.
\begin{table}[h]
%%\label{tableNSL}
   \centering
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
&  $\alpha$ &Gen.Role& $R^-$ & $r^+$ &  Theo. \ref{PAT}\\
  \hline
1&  $k_{ab}^i$ & $A$& $X$ & $\{X.k_{ab}^i\}_{k_{as}}$ & Not Respected\\
  \hline
2& $X$ &  $A$ & $X$ & $\{X.k_{ab}^i\}_{k_{as}}$& Respected\\
  \hline
 \hline
3&  $N_b^i$ & $B$& $A$ & $N_b^i$ & Respected\\
  \hline
4& $Y$ &  $B$ & $Y$ & $\{A.Y \}_{k_{bs}}$& Respected\\
  \hline
 \hline
5&  $U$ & $S$& $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ & $\{U.V\}_{k_{bs}}$ & Respected\\
  \hline
6& $V$ &  $S$ & $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ & $\{U.V\}_{k_{bs}}$& Not Respected\\
 \hline
\end{tabular}
\\\hspace{\linewidth}
\caption[]{\label{WLAMGrowthFaille} Compliance of Woo and Lam protocol with the theorem \ref{PAT}}
\end{table}

From Table \ref{WLAMGrowthFaille}, we conclude that this version of the Woo and Lam protocol is not conform with the correctness criterion stated by the theorem \ref{PAT}. Hence, we cannot conclude that it is growing and therefore we deduce anything with respect to its correctness for the property of secrecy. All that we can deduce is: "If the protocol contains some flaw, it would be because of one of non-growth steps shown in the rows 1  and 6 of Table \ref{WLAMGrowthFaille}". 


\begin{comment}
Along with this, in the literature, we proclaim a flaw in this protocol that operates on the drop of the level of security of the variable $V$ in the generalized role of the server $S$ as described in the row 6 of Table \ref{WLAMGrowthFaille}. Now that we learn that this protocol contains a flaw, we deduce by modus-tollens that: \textit{" This protocol could never be proved growing by any Witness-Function"}.%%The attack scenario is described by Table \ref{WLMV:trace}. Indeed, the server $S$ might receive a message (e.g. the session key $k_{ab}^i$) substituting the variable $V$  in the message $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ such that it is protected by $k_{as}$ only (see 3.3.2), then it sends it encrypted by the key $k_{bs}$ in the message $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$. This encryption was not enough good to ensure its secrecy in this message as shown in 3.6.2. 

 	\begin{table}[!h]
            \begin{center}
            \begin{tabular}{|l|}
            \hline
            \\
                            $step.1.~ A\rightarrow I(B): A$ \\
                            $step.2.~ I(B)\rightarrow A: N_b^{i} $\\
                            $step.3.~ A\rightarrow I(B) :  \{N_b^i.k_{ab}^i\}_{k_{as}}$\\
                            \hspace{0.5cm} $step.4.~ I(B)\rightarrow S : \{A.\{N_b^i.k_{ab}^i\}_{k_{as}}\}_{k_{is}}$\\
                            \hspace{0.5cm} $step.5.~ S\rightarrow I(B) :  \{N_b^i.k_{ab}^i\}_{k_{is}}$\\
            \\
            \hline
            \end{tabular}
            \end{center}
            \caption{\label{WLMV:trace} Flaw of the  Woo-Lam Protocol}
            \end{table}

\end{comment}

==> WooLamFaille2.tex <==
\section*{Analysis of the Woo-Lam Protocol (Falwed Version) using a Witness-Function}\label{sectionAnWL1}
In this section, we run an analysis on the flawed version of the Woo-Lam protocol using the Witness-Function ${{\cal{W}}}_{p,{F}_{MAX}^{EK}}$.
Let us consider the flawed version of the Woo and  Lam   protocol denoted by $p$ and  defined in Table~\ref{WLMV:protv2p}.

\begin {table}[H]
\label{WLMV:protv2p} 
\begin{center}
\begin{tabular}{|ll|}
     \hline
     &\\
                    $p$   =&$\langle 1,A\rightarrow B: A\rangle.$  \\
                    & $\langle 2,B\rightarrow A: N_b\rangle.$ \\
                    & $\langle 3,A\rightarrow B: \{ N_b.k_{ab}\}_{k_{as}}\rangle.$ \\
                    & $\langle 4,B\rightarrow S:\{A.\{N_b.k_{ab}\}_{k_{as}}\}_{k_{bs}}\rangle.$  \\
                    & $\langle 5,S\rightarrow B:\{N_b.k_{ab}\}_{k_{bs}}\rangle$.\\ &\\
                %%    \end{array} \\  
              \hline  
\end{tabular}
\caption{\label{WLMV:protv2p} The Woo and Lam Protocol}
\end{center}
\end {table}


\begin{comment}

          \begin{table}[h]
             %%  \begin{array}{|l|}
              %% 
                   \begin{array}{ll}
                    \hline\\
                    $p$   =&$\langle 1,A\rightarrow B: A\rangle.$  \\
                    & $\langle 2,B\rightarrow A: N_b\rangle.$ \\
                    & $\langle 3,A\rightarrow B: \{ N_b.k_{ab}\}_{k_{as}}\rangle.$ \\
                    & $\langle 4,B\rightarrow S:\{A.\{N_b.k_{ab}\}_{k_{as}}\}_{k_{bs}}\rangle.$  \\
                    & $\langle 5,S\rightarrow B:\{N_b.k_{ab}\}_{k_{bs}}\rangle$\\ &\\
                %%    \end{array} \\  
              \hline  
           \end{array}
         \end{center}
    \caption{\label{WLMV:protv2p} The Woo and Lam Protocol}
         \end{table}
\end{comment}

    The   role-based   specification   is ${\cal R}_G(p) = \{{\cal A}_G ^1,
    ~{\cal  A}_G  ^2,~{\cal B}_G ^1,~{\cal B}_G ^2,~{\cal B}_G ^3,~ {\cal S}_G ^1\}$,
    where the generalized roles ${\cal A}_G ^1$, ${\cal A}_G ^2$, of $A$ are as follows:
    \[\begin{array}{l}
            \begin{array}{lllllll}
                    {\cal A}_G ^1 =& \langle  i.1,&  A    & \rightarrow & I(B)&  :&  A
                    \rangle\\
            \end{array}\\
                    \\
             \begin{array}{lllllll}
                    {\cal A}_G ^2=& \langle  i.1,&  A    & \rightarrow & I(B)&  :&  A \rangle .\\
                    & \langle i.2,&  I(B) & \rightarrow & A   &  :&  X \rangle .\\
                    & \langle i.3,&  A    & \rightarrow & I(B)&  :&  \{X.k_{ab}^i\}_{k_{as}}\rangle
             \end{array}\end{array}\]

     The generalized roles ${\cal B}_G ^1$, ${\cal B}_G ^2$, ${\cal B}_G
    ^3$,  of $B$ are as follows:
            \[\begin{array}{l}
            \begin{array}{lllllll}
                {\cal B}_G ^1=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                        & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b^i \rangle  \\
            \end{array}\\ \\
            \begin{array}{lllllll}
                    {\cal B}_G ^2=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                    & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b ^i\rangle .\\
                    & \langle i.3,&  I(A) & \rightarrow & B   &  :&  Y \rangle .\\
                    & \langle i.4,&  B    & \rightarrow & I(S)&  :& \{A.Y \}_{k_{bs}}\rangle .
            \end{array}\\ \\
            \begin{array}{lllllll}
                    {\cal B}_G ^2=& \langle i.1,&  I(A) & \rightarrow & B   &  :&  A \rangle .\\
                    & \langle i.2,&  B    & \rightarrow & I(A)&  :&  N_b ^i\rangle .\\
                    & \langle i.3,&  I(A) & \rightarrow & B   &  :&  Y \rangle .\\
                    & \langle i.4,&  B    & \rightarrow & I(S)&  :& \{A.Y \}_{k_{bs}}\rangle .\\
                    & \langle i.5,&  I(S) & \rightarrow & B&  :&  \{{N_b^i}.Z\}_{k_{bs}} \rangle \\
            \end{array}
             \end{array}\]

             The  generalized role $ {\cal S}_G ^1$, of $S$ is as follows:
            \[\begin{array}{l}
             \begin{array}{lllllll}
                            {\cal S}_G ^1= & \langle i.4,& I(B) & \rightarrow & S & :&\{A.\{U.V\}_{k_{as}}\}_{k_{bs}} \rangle . \\
                                    & \langle i.5,& S & \rightarrow & I(B)& :& \{U.V\}_{k_{bs}}\rangle\\
               \end{array}
            \end{array} \]
Let us have a context of verification such that: \\
$\ulcorner k_{as}\urcorner=\{A, S\}$; $\ulcorner k_{bs}\urcorner=\{B, S\}$; $\ulcorner k_{ab}^i\urcorner=\{A, B, S\}$; 
$\ulcorner N_b^i \urcorner=\bot$; $\forall A\in {\cal{I}}, \ulcorner A \urcorner=\bot$.\\
The principal identities are not analyzed since they are set public in the context.\\
Let $F\equiv {F}_{MAX}^{EK}$; ${{\mathcal{W}}}_{p,{F}}\equiv {{\mathcal{W}}}_{p,{F}_{MAX}^{EK}}$;\\
We denote  by ${{\mathcal{W}}}_{p,{F}}'(\alpha,m)$ the lower bound: $\underset{\overset {m' \in {\cal{M}}_p^{\cal{G}}}{\exists \sigma' \in \Gamma.m'\sigma' = m\sigma' }}{\sqcap} {F}(\alpha, \partial [\overline{\alpha}]m'\sigma')$ of the witness-function ${{\mathcal{W}}}_{p,{F}}(\alpha,m)$.\\
Let  ${\cal{M}}_p^{\cal{G}}=\{
A_1,
X_1,
\{X_2.k_{A_2 B_1}^i\}_{k_{A_2 S_1}},
A_3,
N_{B_{2}}^i,
Y_1,\\
 \{A_4.Y_1 \}_{k_{B_3 S_2}},
\{{N_{B_4}^i}.Z_1\}_{k_{B_4 S_3}},
\{A_5.\{U_1.V_1\}_{k_{A_5 S_4}}\}_{k_{B_5 S_4}}, \\
\{U_2.V_2\}_{k_{B_6 S_5}}
 \}$\\
After elimination of duplicates,
${\cal{M}}_p^{\cal{G}}=\{
A_1,
X_1,\\
\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}},
N_{B_{2}}^i,
 \{A_4.Y_1 \}_{K_{B_3 S_2}},
\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},\\
\{A_5.\{U_1.V_1\}_{K_{A_5 S_4}}\}_{K_{B_5 S_4}},
\{U_2.V_2\}_{K_{B_6 S_5}}
 \}$\\The variables are denoted by $X_1, X_2,Y_1, Z_1, U_1, U_2, V_1$ and $V_2$;\\ 
The static names are denoted by $A_1$, $A_2$, $B_{1}$, ${K_{A_{2}S_{1}}}$, 
$N_{B_{2}}^i$, $A_4$, ${K_{{B_{3}S_2}}}$, 
$N_{B_{4}}^i$, ${K_{B_{4}S_3}}$, 
$A_5$, ${K_{{A_5}S_4}}$, ${K_{{B_5}S_4}}$ 
 and ${K_{B_{6}S_5}}$.
\subsection{Analysis of the generalized role of $A$}
As defined in the generalized role $A$, an agent $A$ can participate in some session $S^{i}$  in which she receives an unkown message $X$ and sends the message $\{X.k_{ab}^i\}_{k_{as}}$. This is described by the following schema: \[{S^{i}}:\frac{X}{\{X.k_{ab}^i\}_{k_{as}}}\]

\noindent\textbf{-Analysis of the messages exchanged  in the session $S^{i}$:}\\
\\
1- For any $k_{ab}^i$:\\
\\
a- When receiving: $R_{S^{i}}^-=X$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=\top$ (1.0)\\
\\
b- When sending: $r_{S^{i}}^+=\{X.k_{ab}^i\}_{k_{as}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall k_{ab}^i.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall k_{ab}^i.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{X.k_{ab}^i\}_{k_{as}}\sigma' } \}$ \\$=\{(\{X_2.K_{A_2 B_1}^i\}_{K_{A_2 S_1}},\sigma_1'), ( \{A_4.Y_1 \}_{K_{B_3 S_2}},\sigma_2'),$\\$(\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},\sigma_3'),(\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_4')\}$ such that: \\
$$\left\{
    \begin{array}{l}
%%      \sigma_1'=\{X_1 \longmapsto\{X.k_{ab}^i\}_{k_{as}}\}   \\
      \sigma_1'=  \{X_2 \longmapsto X, K_{A_2 B_1}\longmapsto k_{ab}, {K_{A_2 S_1}} \longmapsto {k_{as}}\}\\
      \sigma_2'=  \{X\longmapsto A_4,Y_1 \longmapsto k_{ab}^i, K_{A_2 S_1} \longmapsto k_{as}\}\\
      \sigma_3'=  \{X\longmapsto {N_{B_4}^i},Z_1 \longmapsto k_{ab}^i, K_{B_4 S_3}\longmapsto k_{as}\}\\
      \sigma_4'=  \{U_2\longmapsto X,V_2 \longmapsto k_{ab}^i, K_{B_6 S_5}\longmapsto k_{as}\}\\
    \end{array}
\right.$$
${{\mathcal{W}}}_{p,{F}}'(k_{ab}^i,\{X.k_{ab}^i\}_{k_{as}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.K_{A_2 B_1}^i\}_{K_{A_2 S_1}} \sigma_{1}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{A_4.Y_1 \}_{K_{B_3 S_2}} \sigma_{2}')\sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}} \sigma_{3}') \sqcap$\\$  {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{4}')$\\
$=\{\mbox{renaming the static neighborhood}\}$\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.k_{ab}^i\}_{k_{as}} \sigma_{1}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{A_4.Y_1\}_{k_{as}} \sigma_{2}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{{N_{B_4}^i}.Z_1\}_{k_{as}} \sigma_{3}') \sqcap$\\$ {F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{U_2.V_2\}_{k_{as}} \sigma_{4}')$   \\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(k_{ab}^i,\partial[\overline{k_{ab}^i}] \{X_2.k_{ab}^i\}_{k_{as}}) \sqcap {F}(Y_1,\partial[\overline{Y_1}] \{A_4.Y_1\}_{k_{as}}) \sqcap {F}(Z_1,\partial[\overline{Z_1}] \{{N_{B_4}^i}.Z_1\}_{k_{as}}) \sqcap {F}(V_2,\partial[\overline{V_2}] \{U_2.V_2\}_{k_{as}})$  \\
%%$=\{\mbox{Since } F={F}_{MAX}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(k_{ab}^i,\{k_{ab}^i\}_{k_{as}}) \sqcap {F}(Y_1,\{A_4.Y_1\}_{k_{as}}) \sqcap$\\$ {F}(Z_1,\partial[\overline{Z_1}] \{{N_{B_4}^i}.Z_1\}_{k_{as}}) \sqcap {F}(V_2,\partial[\overline{V_2}] \{V_2\}_{k_{as}})$ \\
$=\{\mbox{Since } F={F}_{MAX}^{EK}\}$\\
$\{ A,  S\} \cup \{A_4, A, S\} \cup \{ A,  S\} \cup \{ A,  S\}=\{A, S, A_4\}$(1.1)\\
\\
2- For any $X$:\\
\\
Since when receiving, we have ${F}(X,\partial  [\overline{X}]X )={F}(X,X)=\bot$, then we have directly:\\
${{\mathcal{W}}}_{p,{F}}'(X,\{X.k_{ab}^i\}_{k_{as}})\sqsupseteq \ulcorner X \urcorner \sqcap {F}(X,\partial  [\overline{X}]X)=\bot$ (1.2)\\
\\
3- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
From (1.1) and (1.2), we have: ${{\mathcal{W}}}_{p,{F}}'(k_{ab}^i,\{X.k_{ab}^i\}_{k_{as}})= \{A, S, A_4\} \not\sqsupseteq \ulcorner k_{ab}^i \urcorner \sqcap {F}(k_{ab}^i,\partial  [\overline{k_{ab}^i}]X )=\{S, A, B\}$ (1.3)\\
From (1.3) we have: the messages exchanged in the session $S^{i}$ (i.e. $k_{ab}^i$) do not respect the correctness criterion stated in the theorem \ref{PAT}. (I)\\


\subsection{Analysis of the generalized role of $B$}
As defined in the generalized roles of $B$, an agent $B$ can participate in two consequent sessions: $S^{i}$ and $S^{j}$ such that $j>i$. In the former session $S^{i}$, the agent $B$ receives the identity $A$ and sends the nonce $N_b ^i$. In the consequent session $S^{j}$, she receives an unknown message $Y$ and she sends the message $\{A.N_b^i.Y \}_{k_{bs}}$. This is described by the following schema:
\[{S^{i}}:\frac{A}{N_b ^i} ~~~~~~~~~~~~~~~~~~~~~~~~ {S^{j}}:\frac{Y}{\{A.Y \}_{k_{bs}}}\]
$ $\\
\textbf{-Analysis of the messages exchanged  in the session $S^{i}$:}\\
\\
1- For any $N_b^i$:\\
Since $N_b^i$ is declared public in the context (i.e. $\ulcorner N_b^i \urcorner=\bot$), then we have directly:\\
${{\mathcal{W}}}_{p,{F}}'(N_b^i,N_b^i)\sqsupseteq \ulcorner N_b^i \urcorner \sqcap {F}(N_b^i,\partial  [\overline{N_b^i}]A )=\bot$ (2.1)\\
\\
\textbf{-Analysis of the messages exchanged  in the session $S^{j}$:}\\
\\
1- For any $Y$:\\
Since when receiving, we have ${F}(Y,\partial  [\overline{Y}]Y )={F}(Y,Y)=\bot$, then we have directly:\\
${{\mathcal{W}}}_{p,{F}}'(Y,\{A.N_b^i.Y \}_{k_{bs}})\sqsupseteq \ulcorner Y \urcorner \sqcap {F}(Y,\partial  [\overline{Y}]Y )=\bot$ (2.2)\\
\\
2- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
From (2.1) and (2.2) we have: the messages exchanged in the session $S^{i}$ and $S^{j}$  respect the correctness criterion stated in the theorem \ref{PAT}. (II)\\

\subsection{Analysis of the generalized role of $S$}
As defined in the generalized role $S$, an agent $S$ can participate in some session $S^{i}$  in which she receives the message $ \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ and sends the message $\{U.V\}_{k_{bs}}$. This is described by the following schema: \[{S^{i}}:\frac{\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}}{\{U.V\}_{k_{bs}}}\]
1- For any $U$:\\
\\
a- When receiving: $R_{S^{i}}^-=\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}} )={F}(U,\{A.\{U\}_{k_{as}}\}_{k_{bs}} )=$\\$(3.1) \left\{
    \begin{array}{ll}
        \{A, B, S\} & \mbox{if } k_{bs} \mbox{ is the external protective}\\
        &\mbox{of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}} (3.1.1)\\
        \\
        \{A, S\} & \mbox{if } k_{as} \mbox{ is the external protective} \\
        &\mbox{of } V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.1.2)
    \end{array}
\right.$ \\
\\
b-When sending: $r_{S^{i}}^+=\{U.V\}_{k_{bs}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall U.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall U.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = \{U.V\}_{k_{bs}} \sigma' } \}$ \\$=\{\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}},\sigma_1'),(,\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_2')\}$ such that: \\
$$\left\{
    \begin{array}{l}
      \sigma_1'=\{ X_2 \longmapsto U,  V \longmapsto k_{A_2 B_1}^i, {K_{A_2 S_1}}\longmapsto  {k_{bs}}\}   \\
      \sigma_2'=\{ U_2 \longmapsto U, V_2\longmapsto V, K_{B_6 S_5}\longmapsto  {k_{bs}}\}  \\
    \end{array}
\right.$$
\\
${{\mathcal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(U,\partial[\overline{U}]\{X_2.k_{A_2 B_1}^i\}_{K_{A_2 S_1}} \sigma_{1}') \sqcap$\\$ {F}(U,\partial[\overline{U}]\{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{2}')$\\
$=\{\mbox{Setting the static neighborhood}\}$\\
${F}(U,\partial[\overline{U}]\{X_2.k_{A_2 B_1}^i\}_{k_{bs}} \sigma_{1}') \sqcap$\\$ {F}(U,\partial[\overline{U}]\{U_2.V_2\}_{k_{bs}} \sigma_{2}')$
\\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(X_2,\partial[\overline{X_2}]\{X_2.k_{A_2 B_1}^i\}_{k_{bs}} \sigma_{1}') \sqcap $\\${F}(U_2,\partial[\overline{U_2}]\{U_2.V_2\}_{k_{bs}} \sigma_{2}')$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(X_2,\{X_2.k_{A_2 B_1}^i\}_{k_{bs}}) \sqcap {F}(U_2,\{U_2\}_{k_{bs}})$ \\
$=\{\mbox{Since } {F}={F}_{MAX}^{EK}\}$\\
$\{B, S\}\cup \{B, S\}=\{B, S\}$(3.2)\\
\\
2- For any $V$:\\
\\
a- When receiving: $R_{S^{i}}^-=\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ \textit{(in a receiving step, the upper bound is used)}\\
${F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})={F}(V,\{A.\{V\}_{k_{as}}\}_{k_{bs}})=$\\$(3.3) \left\{
    \begin{array}{ll}
        \{A, B, S\} & \mbox{if } k_{bs} \mbox{ is the external protective key}\\
        &  \mbox{of } V \mbox{in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.3.1)\\
       \\
        \{A, S\} & \mbox{if } k_{as} \mbox{ is the external protective key} \\
      & \mbox{of } V\mbox{in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.3.2)
    \end{array}
\right.$ \\
\\
b-When sending: $r_{S^{i}}^+=\{U.V\}_{k_{bs}}$ \textit{(in a sending step, the lower bound is used)}\\
 $\forall V.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' = r_{S^{i}}^+\sigma' } \}$\\$=\forall V.\{m' \in {\cal{M}}_p^{\cal{G}}|{\exists \sigma' \in \Gamma.m'\sigma' =\{U.V\}_{k_{bs}} \sigma' } \}$ \\$=\{( \{A_4.Y_1 \}_{k_{B_3 S_2}},\sigma_1'),(\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}},\sigma_2'),$\\$(\{U_2.V_2\}_{K_{B_6 S_5}},\sigma_3')\}$ such that: \\
$$\left\{
    \begin{array}{l}
      \sigma_1'=\{ U \longmapsto A_4, Y_1 \longmapsto V, {K_{B_{3}S_2}}\longmapsto  {k_{bs}}\}   \\
      \sigma_2'=\{ U \longmapsto N_{B_{4}}^i, Z_1 \longmapsto V, {K_{B_{4}S_3}}\longmapsto  {k_{bs}}\}  \\
      \sigma_3'=\{ U_2 \longmapsto U, V_2 \longmapsto V, {K_{B_6 S_5}}\longmapsto  {k_{bs}}\}  \\
    \end{array}
\right.$$
\\
${{\mathcal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})$\\
$=\{\mbox{Definition of the lower bound of the Witness-Function}\}$\\
${F}(V,\partial[\overline{V}] \{A_4.Y_1 \}_{k_{B_3 S_2}}\sigma_{1}') \sqcap$\\${F}(V,\partial[\overline{V}]\{{N_{B_4}^i}.Z_1\}_{K_{B_4 S_3}} \sigma_{2}')\sqcap$\\${F}(V,\partial[\overline{V}]\{U_2.V_2\}_{K_{B_6 S_5}} \sigma_{3}')$\\
$=\{\mbox{Setting the static neighborhood}\}$\\
${F}(V,\partial[\overline{V}] \{A_4.Y_1\}_{k_{bs}}\sigma_{1}') \sqcap {F}(V,\partial[\overline{V}]\{{N_{B_4}^i}.Z_1\}_{k_{bs}} \sigma_{2}')\sqcap {F}(V,\partial[\overline{V}]\{U_2.V_2\}_{K_{bs}} \sigma_{3}')$\\
$=\{\mbox{Definition } \ref{Fder}\}$
\\
${F}(Y_1,\partial[\overline{Y_1}] \{A_4.Y_1\}_{k_{bs}}\sigma_{1}') \sqcap {F}(Z_1,\partial[\overline{Z_1}]\{{N_{B_4}^i}.Z_1\}_{k_{bs}} \sigma_{2}')\sqcap {F}(V_2,\partial[\overline{V_2}]\{U_2.V_2\}_{K_{bs}} \sigma_{3}')$\\
%%$=\{\mbox{Since } F={F}_{MAX}^{EK}\}$\\
$=\{\mbox{Derivation in the definition } \ref{derivation}\}$
\\
${F}(Y_1,\{A_4.Y_1\}_{k_{bs}}) \sqcap {F}(Z_1,\{{N_{B_4}^i}.Z_1\}_{k_{bs}})\sqcap {F}(V_2,\{V_2\}_{K_{bs}})$\\$=\{\mbox{Since } {F}={F}_{MAX}^{EK}\}$\\
$\{ A_4, B, S\}\cup \{ B, S\}\cup \{B, S\}=\{ A_4, B, S\}$(3.4)\\
3- Compliance with the correctness criterion stated in the theorem \ref{PAT}:\\
For any $U$, from (3.1) and (3.2) we have:\\
%%\small{
\\$(3.5)  \left\{
  \begin{array}{ll}
 {{\mathcal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}}\}_{k_{bs}})=\{A, B, S\} \sqsupseteq&\\
\ulcorner U \urcorner \sqcap {F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=      & \\
  \ulcorner U \urcorner \cup  \{A, B, S\} \mbox{ if } k_{bs} \mbox{ is the external protective}& \\
 \mbox{key of }U \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.5.1)&\\
\\
 {{\mathcal{W}}}_{p,{F}}'(U,\{U.V\}_{k_{bs}}\}_{k_{bs}})=\{A, B, S\}\not\sqsupseteq &\\
\ulcorner U \urcorner \sqcap {F}(U,\partial  [\overline{U}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=     &\\
 \ulcorner U \urcorner \cup   \{A, S\} \mbox{ if } k_{as} \mbox{ is the external protective}  &\\
\mbox{key of }   U \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.5.2)&
    \end{array}
\right.$ \\
%%}
\normalsize
$ $\\
For any $V$, from (3.3) and (3.4) we have:\\
%%\small{
\\$(3.6)\left\{
    \begin{array}{lll}
 {{\mathcal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})=\{A_4, B, S\} \not \sqsupseteq & &\\
\ulcorner V \urcorner \sqcap {F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=    &&\\
\ulcorner V \urcorner \cup     \{A, B, S\} \mbox{ if } k_{bs} \mbox{ is the external protective} &&\\
\mbox{key of }  V \mbox{ in }  \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.6.1) &&\\
\\
{{\mathcal{W}}}_{p,{F}}'(V,\{U.V\}_{k_{bs}})=\{A_4, B, S\} \not\sqsupseteq &&\\
\ulcorner V \urcorner \sqcap {F}(V,\partial  [\overline{V}]\{A.\{U.V\}_{k_{as}}\}_{k_{bs}})=     && \\
\ulcorner V \urcorner \cup    \{A, S\}  \mbox{ if } k_{as} \mbox{ is the external protective}   &&\\
\mbox{key of }  V \mbox{ in } \{A.\{U.V\}_{k_{as}}\}_{k_{bs}}(3.6.2) &&
    \end{array}
\right.$ \\
%%}
\normalsize
$ $\\
From (3.5)  and (3.6) we have: the messages exchanged in the session $S^{i}$  do not respect the correctness criterion stated in the theorem \ref{PAT} (III)

\section{Results and Interpretation}

The analysis results of the Woo and Lam protocol are summarized in Table \ref{WLAMGrowthFaille1}.



\begin{table}[h]
%%\caption[]{ Compliance of Woo and Lam protocol with the theorem \ref{PAT}}
\caption{Compliance of Woo and Lam protocol with the theorem \ref{PAT}}
\label{WLAMGrowthFaille1}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
  \hline
&  $\alpha$ &G. Role& $R^-$ & $r^+$ &  Theo. \ref{PAT}\\
  \hline
1&  $k_{ab}^i$ & $A$& $X$ & $\{X.k_{ab}^i\}_{k_{as}}$ & Not Respected\\
  \hline
2& $X$ &  $A$ & $X$ & $\{X.k_{ab}^i\}_{k_{as}}$& Respected\\
  \hline
 \hline
3&  $N_b^i$ & $B$& $A$ & $N_b^i$ & Respected\\
  \hline
4& $Y$ &  $B$ & $Y$ & $\{A.Y \}_{k_{bs}}$& Respected\\
  \hline
 \hline
5&  $U$ & $S$& $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ & $\{U.V\}_{k_{bs}}$ & Not Respected\\
  \hline
6& $V$ &  $S$ & $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ & $\{U.V\}_{k_{bs}}$& Not Respected\\
 \hline
\end{tabular}

\end{center}
\end{table}


\normalsize
From Table \ref{WLAMGrowthFaille1}, we conclude that this version of the Woo-Lam protocol does not respect the correctness criterion stated by the theorem \ref{PAT}. Hence, we cannot conclude anything regarding its correctness with respect to the property of confidentiality. All that we can deduce is: "If the protocol contains a flaw, it would be because of one of non-growth steps shown in the rows 1, 5 and 6 of Table \ref{WLAMGrowthFaille1}". Consistent with this, in the literature, we report a flaw in this protocol that exploits the decay of the level of security of the variable $V$ in the generalized role of the server $S$ as shown in the row 6 of Table \ref{WLAMGrowthFaille1}. The attack scenario is described by Table \ref{WLMV:trace}. Indeed, the server $S$ might receive a message (e.g. the session key $k_{ab}^i$) substituting the variable $V$  in the message $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$ such that it is protected by $k_{as}$ only (see 3.3.2), then he  sends it encrypted by the key $k_{bs}$ in the message $\{A.\{U.V\}_{k_{as}}\}_{k_{bs}}$. This encryption was not enough good to ensure its secrecy in this message as shown in the statement 3.6.2. 

 	\begin{table}[H]
            \begin{center}
            \begin{tabular}{|l|}
            \hline
            \\
                            $\alpha.1.~ A\rightarrow I(B): A$ \\
                            $\alpha.2.~ I(B)\rightarrow A: N_b^{i} $\\
                            $\alpha.3.~ A\rightarrow I(B) :  \{N_b^i.k_{ab}^i\}_{k_{as}}$\\
                            \hspace{0.5cm} $\beta.4.~ I(B)\rightarrow S : \{A.\{N_b^i.k_{ab}^i\}_{k_{as}}\}_{k_{is}}$\\
                            \hspace{0.5cm} $\beta.5.~ S\rightarrow I(B) :  \{N_b^i.k_{ab}^i\}_{k_{is}}$\\
            \\
            \hline
            \end{tabular}
            \caption{Flaw in the  Woo-Lam Protocol}
           \label{WLMV:trace}
            \end{center}
            \end{table}



Now that we know that this protocol contains this flaw, we can conclude by modus-tollens of the the theorem \ref{PAT} the following: " There is no hope to find any Witness-Function such that this protocol would be increasing when analyzed with it".



==> motivation.tex <==
%%\section*{Appendix note}
%%In the appendix, we provide the proofs, a case-study and a brief summary of the context and the notations used all-over this paper.

\section{Introduction}
In this paper, we introduce a new static approach to analyze cryptographic protocols with a new category of functions that we call: the witness-functions, for the property of confidentiality. Intuitively, an increasing protocol preserves the secret. In other words, if the security of any atomic message does not decrease between receiving and sending steps of a protocol, the secret is never leaked. For that, we should define "good"  metrics to evaluate the security of any atomic message. This way of thinking has been considered in some previous works. In~\cite{Schneider4}, Steve Schneider proposed the concept of rank-functions as metrics to analyze protocols in CSP algebra. These functions were successful in analyzing Needham-Schroeder protocol. However, a such analysis requires the protocol implementation in CSP~\cite{Schneider96,SchneiderD04}. Besides, building rank-functions is not a trivial job and their existence is not sure~\cite{Heather}. In~\cite{AbadiTyping} Abadi, using Spi-Calculus~\cite{SPI1,SPI2}, guarantees that: "If a protocol typechecks, then it does not leak its secret inputs". To do so, he requests from the exchanged messages to be composed of four parts having strictly the following types: \{secret, public, any, confounder\} in order to recognize the security level of every part. However, this approach cannot analyze protocols that had been implemented with no respect to this restriction. 
In the same vein, Houmani and al.~\cite{Houmani1,Houmani3,Houmani8,Houmani5} defined universal functions called interpretation functions able to analyze a protocol statically and operate on an abstraction of the protocol  called generalized roles, that generate a space of messages with variables. An interpretation function must meet some sufficient conditions to be reliable for the analysis. Obviously, less we have conditions on functions, more we have functions and more we have chance to get protocols proved correct since one function may fail to prove the growth of a protocol but another may manage to do. However, we notice that the conditions on functions were so restrictive that only two concrete functions had been proposed. 
We believe that the condition related to the full-invariance by substitution, which is the property-bridge between an analysis run on messages of the generalized roles and the conclusion made on valid traces, is the most restrictive one.
Since the aim of our approach is to build as many reliable functions as we are able to do, we think that if we free a function from this restrictive condition, we can build more functions. Nevertheless, freeing a function from a condition may impel us to take additional precautions. In this work, we present the witness-functions %%~\cite{WitnessArt1,WitnessArt2,WitnessArt3} 
to analyze cryptographic protocols.  We show how to build them. We show that a witness-function offers two bounds that allow us to get rid of the restrictive condition of full-invariance by substitution in Houmani's work by using derivation techniques. We state then the theorem of protocol analysis with the Witness-Functions that sets an interesting criterion for the protocol correctness. Finally, we run an analysis on the  correct version of the Woo and Lam protocol.


